What You Don't Know Can Hurt You: Use and Abuse of Astrophysical Models in Gravitational-wave Population Analyses

One of the goals of gravitational-wave astrophysics is to infer the number and properties of the formation channels of binary black holes (BBHs); to do so, one must be able to connect various models with the data. We explore benefits and potential issues with analyses using models informed by population synthesis. We consider 5 possible formation channels of BBHs, as in Zevin et al. (2021b). First, we confirm with the GWTC-3 catalog what Zevin et al. (2021b) found in the GWTC-2 catalog, i.e. that the data are not consistent with the totality of observed BBHs forming in any single channel. Next, using simulated detections, we show that the uncertainties in the estimation of the branching ratios can shrink by up to a factor of $\sim 1.7$ as the catalog size increases from $50$ to $250$, within the expected number of BBH detections in LIGO-Virgo-KAGRA's fourth observing run. Finally, we show that this type of analysis is prone to significant biases. By simulating universes where all sources originate from a single channel, we show that the influence of the Bayesian prior can make it challenging to conclude that one channel produces all signals. Furthermore, by simulating universes where all 5 channels contribute but only a subset of channels are used in the analysis, we show that biases in the branching ratios can be as large as $\sim 50\%$ with $250$ detections. This suggests that caution should be used when interpreting the results of analyses based on strongly modeled astrophysical sub-populations.

==> referee_report.tex <==
Reviewer:
In this work, the authors study the impact of using population synthesis-informed models on inferences about the population properties of binary black holes. They explore five possible formation channels of binary black holes, finding the latest catalogue of gravitational wave events (GWTC-3) to not be consistent with just a single formation channel. This work also highlights the importance of taking caution when making inferences on the population using these models, and the biases that can be introduced if the model does not represent the true astrophysical distribution. The paper is well written and provides a detailed explanation of the methods and results. I would recommend the acceptance of this paper. I have some minor comments and questions for the authors to consider.

1) The authors indicate they used only the 'confident BBH' in the catalogue which I believe means that event GW190814 was not included? If so, it would be good to explicitly mention that. How would including this event impact your inferences given it is quite a unique event?

2) Is there a reason you chose to focus on 'values of the common envelope efficiency, quasi-isolated natal black hole spins, and branching ratios' for the simulated catalogues and not any other parameters? Do they have the largest impact?

3) The authors mention that they "use an uninformative prior for the hyperparameters" Perhaps this phrase could be cut (since the prior information is mentioned directly after) or reworded to say something like "a broad prior to cover the parameter space" to avoid using the word 'uninformative'?

4) Figure 8 would benefit from less axis ticks for legibility (if it remains a single column plot).

5) In Figure 12, could the authors include a description in the caption as well on why alpha_CE 1.0 and 0.5 plots are populated for a universe with a universe of alpha_CE 1.0, and the blank panels for chi_beta = 0? This way the plot can be understood in isolation.

---
The ApJ statistics editor made the following additional comment on your work, which you should treat in the same way as reviewer comments:

The authors may find it useful that there is a well-accepted level of Bayes factors for model selection purposes. Model A is preferred over Model B if \Delta(BIC)>8-10. This threshold is proposed by distinguished statisticians Kass & Raftery (www.jstor.org/stable/2291091, 19K citations).

==> referee_response.tex <==
We thank the referee for a thoughtful report. We agree with all of the points brought up by the referee, and have accordingly updated the manuscript. Each comment is responded to inline below, with our responses marked with (R). Changes in the manuscript have also been colored red and boldfaced for clarity. 

Reviewer:
In this work, the authors study the impact of using population synthesis-informed models on inferences about the population properties of binary black holes. They explore five possible formation channels of binary black holes, finding the latest catalogue of gravitational wave events (GWTC-3) to not be consistent with just a single formation channel. This work also highlights the importance of taking caution when making inferences on the population using these models, and the biases that can be introduced if the model does not represent the true astrophysical distribution. The paper is well written and provides a detailed explanation of the methods and results. I would recommend the acceptance of this paper. I have some minor comments and questions for the authors to consider.

1) The authors indicate they used only the 'confident BBH' in the catalogue which I believe means that event GW190814 was not included? If so, it would be good to explicitly mention that. How would including this event impact your inferences given it is quite a unique event?

(R) We thank the referee for pointing this out, as we forgot to mention GW190814 in our manuscript. As with GW190521, none of our models have support for mass ratios as asymmetric as GW190814, and opt to exclude it from our analysis. Furthermore, the interpretation of this event as a BBH is uncertain, as there are no astrophysical models that can unambiguously explain GW190814. We added two sentences in the first paragraph of Section 2.2 clarifying this. 

2) Is there a reason you chose to focus on 'values of the common envelope efficiency, quasi-isolated natal black hole spins, and branching ratios' for the simulated catalogues and not any other parameters? Do they have the largest impact?

(R) We agree with the referee that there are many other uncertain physical parameters that could be considered in an analysis such as this. The reason for focusing on the common envelope efficiencies and quasi-isolated black hole spins are based on the astrophysical models that were available across the different formation channels we explored. The most computationally expensive models to run are the globular cluster models using the Cluster Monte Carlo (CMC) code. We used the globular cluster models from Rodriguez et al. 2019 (https://ui.adsabs.harvard.edu/abs/2019PhRvD.100d3027R/abstract), which explore the 4 discrete spin variations also considered in our work. Considering additional values of the natal spin cannot be accomplished in post-processing for the cluster models, since the natal spin of black holes has a significant impact on the retention of BBH merger products in clusters, and thus affect the evolution of the cluster as a whole. Choosing the common envelope efficiency as the second parameter to explore was due to this parameter only affecting one of the five astrophysical models considered in this work, and thus only requiring additional models in addition to the spin variations for one of the five formation channel models. Note that if another parameter was chosen that affects all five formation channels rather than the common envelope efficiency, we would require 100 distinct astrophysical models rather than 36. We comment on why common envelope efficiencies and quasi-isolated black hole spins are the focus of this work in a newly-added footnote (footnote 2). 

3) The authors mention that they "use an uninformative prior for the hyperparameters" Perhaps this phrase could be cut (since the prior information is mentioned directly after) or reworded to say something like "a broad prior to cover the parameter space" to avoid using the word 'uninformative'?

(R) We have replaced the word 'uninformative' with 'broad and agnostic'. 

4) Figure 8 would benefit from less axis ticks for legibility (if it remains a single column plot).

(R) The plot has been updated with axis ticks pointing inwards, which should improve legibility.

5) In Figure 12, could the authors include a description in the caption as well on why alpha_CE 1.0 and 0.5 plots are populated for a universe with a universe of alpha_CE 1.0, and the blank panels for chi_beta = 0? This way the plot can be understood in isolation.

(R) A corresponding description has been included such that the plot can be read in isolation.

---
The ApJ statistics editor made the following additional comment on your work, which you should treat in the same way as reviewer comments:

The authors may find it useful that there is a well-accepted level of Bayes factors for model selection purposes. Model A is preferred over Model B if \Delta(BIC)>8-10. This threshold is proposed by distinguished statisticians Kass & Raftery (www.jstor.org/stable/2291091, 19K citations).

(R) We have added a sentence in Section 2.1 to help the reader interpret Bayes factors, citing Kass & Raftery 1995. 

---
Finally, although this change was not suggested by the referee, we have added a sentence in Section 4.1 that explicitly refers to the prior curves in Figure 6 when discussing the prior bias against a single dominating channel.




